Deepfakes, Phrenology, Surveillance, and More! A Taxonomy of AI Privacy Risks

Privacy is a key principle for developing ethical AI technologies, but how does including AI technologies in products and services change privacy risks? We constructed a taxonomy of AI privacy risks by analyzing 321 documented AI privacy incidents. We codified how the unique capabilities and requirements of AI technologies described in those incidents generated new privacy risks, exacerbated known ones, or otherwise did not meaningfully alter the risk. We present 12 high-level privacy risks that AI technologies either newly created (e.g., exposure risks from deepfake pornography) or exacerbated (e.g., surveillance risks from collecting training data). One upshot of our work is that incorporating AI technologies into a product can alter the privacy risks it entails. Yet, current approaches to privacy-preserving AI/ML (e.g., federated learning, differential privacy, checklists) only address a subset of the privacy risks arising from the capabilities and data requirements of AI.

==> sections/_archived__1-introduction.tex <==
\section{Introduction}
% TODO
% - 

% The state of the world
% - incorporating AI into technologies is a trend that is happening in multiple sectors
% - however, we also see various privacy incidents when these AI technology deployed in the real world (give some AI incident examples here)
% - existing RAI framework sees privacy as one of the core RAI principles
% - few tools were created to design for privacy
% - vague compliance for AI practitioners privacy practices (our under review FAccT paper)
% - privacy suggestions remain very high level
% For better or worse, AI technologies are here to stay. New AI technologies are constantly created and evolving, and so do their harms to individuals and society \cite{pownall_ai_2023}. Behavioral advertising, for example, in which users’ interests are inferred from their behaviors online to target them with relevant advertisements —-- can be perceived by users as both ``smart'' and ``scary'' \cite{ur_smart_2012}. Systems of the same concept have also been implemented in the physical world, whose cameras were installed with facial recognition capability to understand the customers \cite{noauthor_xpeng_nodate}. On the other hand, a class of ``AI physiognomy'' applications such as predicting one's sexual orientation \cite{} and criminality \cite{} from a picture of an individual’s face, have also been widely researched and deployed.

% In response to the potential detrimental effects of unchecked AI on society, responsible AI (RAI) --- an approach to AI research and practice that centers human needs, societal good and safety \cite{} —-- has emerged as a rebuttal to traditional approaches to AI research.
% In the past few years, individuals and institutions spanning governments, professional societies, academia and industry have proposed guidelines and principles for RAI to equip AI practitioners who design and create AI technologies with tools and approaches to make AI more ethical and responsible \cite{}. Unsurprisingly, privacy was found to be one of the five most commonly mentioned principles in a recent meta-review of published RAI guidelines \cite{jobin_global_2019}. However, ``the gap between principles and practice'' was also found to remain significant \cite{}, and such a gap can be especially prominent for consideration of end-user privacy in the design of AI technologies.

In recent years, institutions spanning governments, academia, and industry have proposed guidelines for human-centered AI (HAI) to make AI more ethical and responsible \cite{li2018make,riedl2019human,shneiderman2020bridging}. A recent review of 84 such guidelines surfaced that privacy is one of the five most frequently cited principles for creating ethical AI \cite{jobin_global_2019}.
However, recent studies have found that few tools exist to help AI practitioners design for privacy when creating AI products \cite{yurrita_towards_2022}, suggesting that AI practitioners may need to rely on non-AI-specific tools and processes in their privacy work.
Thus, there is a plausible need for more AI-specific privacy design guidance for practitioners. 
We position this work as the first step in adapting standard product privacy guidance to AI-specific guidance by codifying whether and how AI fundamentally changes the landscape of privacy intrusions.

% For example, privacy has long been considered a ``secondary concern'' in product development and require external function such as compliance to motivate such initiatives \cite{}. That said, privacy compliance has been found to be too vague for practitioners to follow through directly \cite{}. Moreover, when AI technologies and their uses led to new perspectives on privacy, few tools have been created to help practitioners design for privacy when creating AI products \cite{yurrita_towards_2022}.

Specifically, the literature currently falls short of a systematic understanding of the privacy intrusions entailed by AI technologies and how such intrusions relate to the unique capabilities and data requirements of AI. Bridging this gap is essential to adequately support AI practitioners in designing for privacy because privacy is notoriously hard to define \cite{goos_privacy_2001,solove_taxonomy_2006} and needs to be contextualized within specific domains to create meaningful and operationalizable solutions (e.g., \cite{goos_privacy_2001}). 
Prior work has attempted to broadly identify and understand different kinds of privacy violations in the context of computing, such as surveillance and identification intrusions \cite{solove_taxonomy_2006}. However, this general approach does not account for the unique capabilities AI technologies offer. 

\begin{figure}[]
\centering
\includegraphics[width=0.7\columnwidth]{figures/overview2.png}
% \vspace{-7mm}
\caption{In this paper, we show if and how AI's unique capabilities and requirements create (purple) and exacerbate (orange) known privacy intrusions entailed by AI technologies.}
\label{fig:overview}
\vspace{-4mm}
\end{figure}

For example, AI can \textit{recommend} courses of action, \textit{infer} users' interests and attributes, and \textit{detect} rare or anomalous events \cite{google2019people}.
In light of the capabilities and potential of AI, the community has also sought ways to engage ``AI as a design material,'' actively exploring how AI can be used to innovate product design \cite{yildirim_how_2022}.
However, these unique capabilities can also entail unique privacy intrusions --- they require the collection, aggregation, and processing of vast troves of personal data (e.g., \cite{mcdonald_clearviews_2020}), they can infer sensitive information about users that they would rather keep hidden (e.g., \cite{levin_new_2017}), and they can be used to predict future events about users that are unsettling (e.g., \cite{jemio_case_2022}).

Simultaneously, there is a great deal of hype surrounding the capabilities and potential of AI, necessitating a critical analysis to differentiate lived harms from speculation.
% Indeed, AI does not change the ways in which end-user privacy is violated altogether. For example, systems infused with AI technologies, as with any other computing technologies, suffer from data leakage due to inadequate security practices (e.g., \cite{turton_hackers_2021}), and data shared with third parties without consent (e.g., \cite{wakefield_location_2021}).
% BUT
% - While AI has its unique capability/ requirement, the existing efforts when defining privacy in AI do not really emphasize such unique characteristics (rather, they treat AI technology as general computing products)
% - What is challenging about defining privacy in AI? (tbd)
%     - you know when you see it; we need empirical evidence of documented intrusions (Solove)
% - This is, in part, because we do not know: how does AI change privacy? How do privacy incidents in AI technologies relate to AI?
% - lower the bar to use AI in products -> more AI capability will be used in AI products
In this work, we shed light on the privacy concerns practitioners should consider about AI by codifying the practical, lived privacy harms that AI technologies pose, and explore whether and how they can be distinguished from non-AI technologies.
% That said, AI does not, and cannot, change the ways in which end-user privacy is violated altogether. For example, systems infused with AI technologies, as with any other computing technologies, suffer from data leakage due to inadequate security practices (e.g., \cite{turton_hackers_2021}), and data shared with third parties without consent (e.g., \cite{wakefield_location_2021}).
We ask: \textbf{How do AI/ML technologies create new and/or exacerbate known end-user privacy intrusions?}


% Thus, we did
% - We construct a taxonomy of privacy infringements and harms entailed by AI technologies. We start with deductive coding on privacy intrusions of reported AI incidents; We then inductively expand and relate each intrusion with AI’s unique capability and requirement.
% - in total, we identify X types of intrusions from X AI incidents with privacy intrusions from AIAAIC
We drew on the AI, Algorithmic and Automation Incident and Controversy Repository (AIAAIC) \cite{pownall_ai_2023} to analyze \totalcase documented AI privacy incidents.
% and contributed a taxonomy of practical, realized privacy intrusions entailed by AI technologies. 
% key findings
Rooting our analysis on Solove's taxonomy of privacy \cite{solove_taxonomy_2006}, we introduce a taxonomy of practical AI privacy intrusions entailed by AI technologies.
We show that the unique capabilities and data requirements of AI can create new and exacerbate known privacy intrusions across nine high-level categories, including surveillance, identification, aggregation, secondary use, exclusion, insecurity, exposure, disclosure, and distortion (see Figure \ref{fig:overview}).
% We further relate each high-level privacy intrusion with the unique capabilities and requirements of AI (see Figure \ref{fig:overview}). 
We found that the unique capabilities of AI create new types of privacy intrusions (e.g., the generation of deepfake pornography creates new exposure intrusions \cite{noauthor_deepfake_2021}), while the data requirements of AI can exacerbate known intrusions (e.g., the collection of face scans in airports create new surveillance intrusions \cite{fassler_south_2021}).

% We define AI technologies as \TODO{XXX}, and see privacy intrusions as \TODO{XXX}.

% The contributions of this work are
This paper makes the following contributions: 
\begin{itemize}
    \item We codified a corpus of \totalcase documented AI incidents and present a taxonomy of privacy infringements created and/or exacerbated by the capabilities and data requirement of AI technology.
    \item Drawing from our taxonomy, we outline ways to aid practitioners in negotiating the utility-intrusiveness trade-off of AI-powered products and services with AI-specific privacy guidance.
\end{itemize}

==> sections/archived_texts.tex <==
% \begin{table}[]
% \centering
% \caption{Cohen's Kappa for each privacy risk}
% \label{tab:irr}
% \resizebox{0.3\textwidth}{!}{
% \begin{tabular}{@{}cc@{}}
% \toprule
% \textbf{Privacy Risk} & \textbf{Cohen's Kappa} \\ \midrule
% Surveillance               & 0.88           \\
% Identification             & 0.94           \\
% Secondary Use              & 0.84          \\
% Aggregation                & 0.87          \\
% Phrenology/Physiognomy    &   1 \\
% Exclusion                  & 0.90           \\
% Insecurity                 & 0.94           \\
% Exposure                   & 1              \\
% Disclosure                 & 1              \\
% Distortion                 & 1              \\
% Increased Accessibility                 & 1               \\
% Intrusion                  & 0.94  
% \\ \bottomrule
% \end{tabular}
% }
% \end{table}




% \begin{table*}
% \renewcommand{\arraystretch}{1.1}
% \centering
% \caption{Taxonomy of AI Privacy Risks}
% \label{tab:taxonomy}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|} 
% \hline
% \textit{\textbf{Privacy intrusions \cite{solove_taxonomy_2006}}}                                                                                                                                                           & \textit{\textbf{How does AI influence privacy~}\textbf{intrusion?}}                                                                                                                                                                                                            & \textit{\textbf{Examples}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ 
% \hline
% \multicolumn{3}{|c|}{\textit{\textbf{Data Collection Intrusions}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Surveillance:\\ \textit{watching, listening to, or}\\ \textit{recording of an individual’s}\\\textit{activities}\end{tabular}                                                                 & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{exacerbates}} surveillance intrusions by\\increasing the scale and ubiquity of personal\\data collected.\end{tabular}                                                                                                                              & \begin{tabular}[c]{@{}l@{}}A predictive policing platform deployed in Xinjiang, China,\\ \textit{``collects [individual's] information from a variety of sources}\\ \textit{including CCTV cameras and Wi-Fi sniffers, as well as}\\ \textit{existing databases of health information, banking records,}\\ \textit{and family planning history''} \cite{rajagopalan_china_2018}.\end{tabular}                                                                                                                                                                                                                                        \\ 
% \hline
% \multicolumn{3}{|c|}{\textit{\textbf{Data Processing Intrusions}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Identification: \\ \textit{linking specific data points}\\ \textit{to an individual’s identity}\end{tabular}                                                                         & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{creates}} new types of identification\\ intrusions with respect to scale, latency, \\robustness, and ubiquity.\end{tabular}                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Models trained on Simulated Masked Face Recognition\\ Dataset (SMFRD) are capable of identifying persons with\\ a mask on, \textit{``violating the privacy of those who wish to}\\ \textit{conceal their face''}\cite{wiggers_ai_2021}.\end{tabular}                                                                                                                                                                                                                                                                                                                                   \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Aggregation:\\ \textit{combining of various pieces}\\ \textit{data about a person to}\\ \textit{make inferences beyond}\\ \textit{what is explicitly captured}\\ \textit{in those data}\end{tabular}         & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{creates}} new types of aggregation \\intrusions owing to their scale, latency, \\ubiquity, and their ability to forecast end-\\user behavior and infer end-user attributes.\end{tabular}                                                               & \begin{tabular}[c]{@{}l@{}} \textit{``The system, called the National Data Analytics Solution}\\ \textit{(NDAS), uses a combination of AI and statistics to try to}\\ \textit{assess the risk of someone committing or becoming a victim}\\\textit{of gun or knife crime"}\cite{baraniuk_exclusive_2018}.\end{tabular}                                                                                                                                                                                                                                                                                                            \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Secondary Use:\\ \textit{the use of personal data}\\ \textit{collected for one purpose}\\ \textit{for a different purpose}\\ \textit{without end-user consent}\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{exacerbates}} secondary use intrusions by \\creating new AI capabilities with collected \\personal data, and (re)creating models from \\a public dataset.\end{tabular}                                                                             & \begin{tabular}[c]{@{}l@{}}The Diversity in Faces (DiF) dataset was created to\\ improve the research on fairness and accuracy of artificial\\ intelligence face recognition systems across genders and\\ skin colors, and should not be used for commercial purposes.\\Nevertheless, two tech giants Amazon and Microsoft\\were accused of using the dataset to \textit{``improve the}\\ \textit{accuracy of their facial recognition software''} \cite{anne_long_amazon_2021}.\end{tabular}                                                                                                                                      \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Exclusion:\\ \textit{data isn’t revealed to the}\\ \textit{person it was collected} \\
% \textit{from or used for}\end{tabular}                                                                 & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{exacerbates}} exclusion intrusions by\\training on rich personal data without consent.\end{tabular}                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}The Large-scale Artificial Intelligence Open Network\\(LAION) is a German non-profit organization that aims \textit{``to}\\ \textit{make large-scale machine learning models, datasets and}\\ \textit{related code available to the general public."} However, a\\ person found out her private medical photographs were\\ referenced in the public image-text dataset, which she\\ \textit{``suspected that someone stole the image from my deceased}\\ \textit{doctor's files and it ended up somewhere online, and then}\\ \textit{it was scraped into this dataset"} \cite{edwards_artist_2022}.\end{tabular}              \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Insecurity:\\ \textit{carelessness in protecting}\\ \textit{collected personal data}\\ \textit{from leaks and improper}\\ \textit{access due to faulty data}\\ \textit{storage and data practices}\end{tabular} & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{exacerbates}} insecurity intrusions by \\introducing new vulnerabilities when\\ incorporating AI and its associated data \\pipeline in the products.\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Lee Luda, a chatbot trained on real-world text conversations,\\ was found to expose the names, nicknames, and home\\ addresses of the users whose data on which it was trained in\\ its responses \cite{jang_south_2021}.\end{tabular}                                                                                                                                                                                                                                                                                                                            \\ 
% \hline
% \multicolumn{3}{|c|}{\textit{\textbf{Data Dissemination Intrusions}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Exposure:\\ \textit{revealing of sensitive}\\ \textit{private information that }\\ \textit{people view as deeply }\\
% \textit{primordial, and that we } \\ 
% \textit{have been socialized into}\\
% \textit{concealing}
% \end{tabular}                                                      & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{creates}} new types of exposure intrusions\\ through generative techniques that can \\create, reconstruct, and manipulate content.\end{tabular}                                                                                                     & \begin{tabular}[c]{@{}l@{}}TecoGAN, a deep learning video clarification tool, could\\clarify censored, pixellated genitalia in videos \cite{montgomery_man_2021}.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Distortion:\\ \textit{disseminating false or}\\ 
% \textit{misleading information}\\ \textit{about individuals that}\\ 
% \textit{impacts the way others}\\
% \textit{judge their character}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{creates}}
% new types of distortion\\
% intrusions through the generation of realistic\\
% fake images and audio that humans have\\
% difficulty discerning as fake.
% \end{tabular}                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}In 2022, the chief communications officer of Binance alleged \\that a \textit{``sophisticated hacking team''} used video footage of his \\previous TV appearances to train an AI hologram of himself~\\for a cryptocurrency scam \cite{vincent_binance_2022}.\end{tabular}                                                                                                                                                                                                                                                                                                   \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Disclosure:\\ \textit{revealing of hidden}\\ 
% \textit{personal information}\\ 
% \textit{about a person that}\\ 
% \textit{impacts the way others }\\ \textit{assess their character}\end{tabular}            & \begin{tabular}[c]{@{}l@{}}AI \textbf{\textit{creates}} new types of disclosure\\
% intrusions by being able to derive or infer\\
% additional information beyond what is\\
% explicitly captured in the raw data.\\ \\ AI \textbf{\textit{exacerbates}} disclosure intrusions through \\sharing personal data to train ML models.\end{tabular} & \begin{tabular}[c]{@{}l@{}}In Shenzhen, China, a system was implemented to detect\\ pedestrians' jaywalking and other offenses captured by\\cameras. The system identifies offenders and displays their\\ photographs, names, and social identification numbers on\\ LED screens placed at road junctions \cite{xu_chinese_2018}.\\ \\ To build a model to detect the risk of patients developing\\ acute kidney injury, the UK’s National Health Service\\ collaborated with Google and shared the mental health\\ records and HIV diagnoses of 1.6 million patients \cite{hal_hodson_revealed_2016}.\end{tabular}  \\
% \hline
% \end{tabular}
% }
% \end{table*}

\subsection{Mitigating privacy risks created and exacerbated by AI}
\label{sec:mitigate AI privacy}
% - the fact that the current tools fall short of identifying and addressing AI privacy risks
% - our taxonomy can be seen as a living structure and can be expended
% - provide research agenda on how we can create AI-specific privacy tools; how we can better consider future AI privacy risks

% Given that AI creates new types of privacy risks and exacerbates existing ones, it follows that there must be a need to provide practitioners with AI-specific product privacy guidance. Without this guidance, AI-created risks are unlikely to be addressed through standard operating procedures.

\textcolor{blue}{
Given that our findings show that AI creates new types of privacy risks and exacerbates existing ones, and that current privacy-preserving AI/ML methods fall short of identifying and addressing many of these risks (Section~\ref{sec:privacy-preserving AI}),
there is a need for future work to fill the gap of mitigating privacy risks created and exacerbated by AI.
To that end, we outline an agenda for future research on 1) creating a living structure for AI privacy risks, and 2) providing practitioners with AI-specific product privacy guidance.}

% Firstly, our taxonomy can serve as the first step to show how common AI requirements and capabilities map onto high-level privacy risks during the product development process. Future work can take an iterative approach, grounded on practitioners' actual design needs, to model the translation function between AI product ideas and potential risks to consider.
% Indeed, envisioning with AI --- i.e., treating AI as a product design material \cite{yang_investigating_2018,jansen_mix_2023,yildirim_how_2022,yildirim_creating_2023} --- is an open and active area of research. Aligning with this line of research, future work can add to our taxonomy by systematizing AI capabilities and requirements, and the privacy risks they create and exacerbate, at a level of granularity that is useful for practitioners to ideate, communicate, and collaborate with product teams and stakeholders \cite{yildirim_how_2022,yildirim_creating_2023}. 


\subsubsection{\textcolor{blue}{Creating a living taxonomy of AI privacy risks}}
\textcolor{blue}{
To our knowledge, our taxonomy is the first attempt to show how common AI requirements and capabilities map onto high-level privacy risks. As shown in Section~\ref{sec:theoretical ai privacy harms}, future AI privacy incidents can also expand the taxonomy.
In addition, future AI privacy incidents may create new categories of privacy risk that go beyond Solove's taxonomy (like the physiognomy risk we describe here). For example, many artists have been vocal about concerns about the theft of artistic style by generative AI \cite{knibbs_new_2023}. While these discussions currently center around notions of copyright and intellectual property, we can envision new types of privacy risk as well: e.g., artistic styles might contain personally identifiable information, as well.
We envision that our taxonomy can complement ongoing crowd-sourced efforts at curating and organizing AI incidents such as the AIAAIC \cite{pownall_ai_2023} and AIID\footnote{\url{https://incidentdatabase.ai/}} by providing a framework to formally synthesize and identify emerging privacy risks in AI incidents. 
With that in mind, the research team is building an interactive interface to present our taxonomy of AI privacy risks, and to collect and aggregate submissions of new incidents related to these risks.
}

\textcolor{blue}{
To present the AI privacy taxonomy in forms useful to the HCI and AI communities, future work can take an iterative approach, grounded on practitioners' and academics' 
actual design and research needs, to model the translation function between AI technology ideas and potential risks to consider.
Indeed, envisioning with AI --- i.e., treating AI as a design material \cite{yang_investigating_2018,jansen_mix_2023,yildirim_how_2022,yildirim_creating_2023} --- is an open and active area of research.
Aligning with this line of research, future work can add to our taxonomy by systematizing AI capabilities and requirements, and the privacy risks they create and exacerbate, at a level of granularity that is useful for practitioners and researchers to ideate, communicate, and collaborate with product teams and stakeholders \cite{yildirim_how_2022,yildirim_creating_2023}.}

\subsubsection{\textcolor{blue}{Creating AI-specific privacy guidance}}
\textcolor{blue}{
Our taxonomy opens up a new design space for privacy-preserving AI/ML tools that aim to raise practitioners' awareness of utility-intrusiveness trade-offs of their AI product ideas (e.g., \cite{ernala_exploring_2021}). 
}
% Specifically, based on our taxonomy, future work can explore approaches to understanding  AI utility-intrusiveness trade-offs when creating AI products (e.g., \cite{ernala_exploring_2021}). 
For example, prior work in other AI-adjacent fields, such as Robotics, has explored how to correlate desired robot function with a minimally-invasive set of sensors \cite{eick_enhancing_2020}.
In the broader context of implementing privacy and security in software products, prior work has found that practitioners still largely see privacy and security in products as an ``all or nothing'' notion such that privacy comes at the expense of other important objectives \cite{tahaei_privacy_2021,gutfleisch_how_2022}. 

\textcolor{blue}{
Future work can explore incorporating our AI privacy taxonomy into harm-envisioning techniques, such as Consequence Scanning \cite{doteveryone_consequence_2020}, by providing AI privacy risk prompts to capture associated negative consequences holistically.
These techniques can help practitioners run lightweight privacy evaluations on AI product ideas, as well as help them balance the utility and intrusiveness of these products and services across design iterations.
With such a tool, we hypothesize that practitioners can better advocate and design for privacy in working contexts that may dissuade this work \cite{tahaei_privacy_2021,lee2024}.
}

Our taxonomy can also consolidate promising future research in foregrounding tensions across data pipelines, practices, and stakeholders (i.e., data subjects, data observers, data beneficiaries, and data victims).
By mirroring the first step in Rahwan's Society in the Loop framework \cite{rahwan_society---loop_2018}, AI practitioners can make concrete the envisioned value and the stakeholders of their proposed AI concepts. 
To assist in this process, future work can create artifacts that encourage practitioners to articulate the value proposition of their envisioned product.
\textcolor{blue}{
Based on our taxonomy, then, it may be possible to mine our database for AI privacy incidents about products that are ``semantically'' similar based on an articulated value proposition.
By showing practitioners related AI privacy incidents, they might then be guided to reflect on the utility-intrusiveness trade-off of their envisioned AI product ideas: 
for whom that value is generated (i.e., data beneficiaries), whose data is processed to unlock that value (i.e., data subjects), who can be impacted by the data pipeline (i.e., data victims), and by which privacy risk (e.g., surveillance).
}

% Ideally, the tool should help practitioners assess the AI utility-intrusiveness trade-off \cite{ernala_exploring_2021} of an AI technology concept by incorporating the perspectives of all data stakeholders.

In practice, however, this type of early-stage discussion around AI utility and privacy risk can be challenging because: (i) practitioners do not necessarily understand the full potential and limitations of AI \cite{yildirim_how_2022}; (ii) privacy is often treated as compliance with general regulatory mandates rather than a product-specific design choice \cite{waldman_designing_nodate}; and, (iii) practitioners do not have access to AI-specific tools that support their privacy work pertaining to the capabilities and requirements that AI brings to their products \cite{lee2024}. Accordingly, there is a need for a greater understanding of where such tools and artifacts might be effectively incorporated into practitioners' workflows.

